Sample Complexity of Data-driven Multistage Stochastic Programming under Markovian Uncertainty

This work is motivated by the challenges of applying the sample average approximation (SAA) method to multistage stochastic programming with an unknown continuous-state Markov process. While SAA is widely used in static and two-stage stochastic optimization, it becomes computationally intractable in general multistage settings as the time horizon $T$ increases. Indeed, the number of samples required to obtain a reasonably accurate solution grows exponentially$\text{ -- }$a phenomenon known as the curse of dimensionality with respect to the time horizon. To overcome this limitation, we propose a novel data-driven approach, the Markov Recombining Scenario Tree (MRST) method, which constructs an approximate problem using only two independent trajectories of historical data. Our analysis demonstrates that the MRST method achieves polynomial sample complexity in $T$, providing a more efficient alternative to SAA. Numerical experiments on the Linear Quadratic Gaussian problem show that MRST outperforms SAA, addressing the curse of dimensionality.

==> old_tex_file/proof.tex <==
We assume the relatively complete recourse and uncertainty set $\Xi_{\mathrm{t}}$ is compact.
Thus, $Q\left(x_{t-1}, \xi_{t}\right)$ is $L_{t}$-Lipschitz continuous in $x_{t-1}$ for $t=2, \ldots, T$.
i. e. , For $t=2, \ldots, T$,
For any fixed $\xi_{t} \in \Xi_{t}$, there exists a constant $L_{t}$ such that
$$
\left|Q_{t}\left(x_{t-1}, \xi_{t}\right)-Q_{t}\left(x_{t-1}^{\prime}, \xi_{t}\right)\right| \leq L_{t}\left\|x_{t-1}-x_{t-1}^{\prime}\right\|, \quad \forall x_{t-1}, x_{t-1}^{\prime} \in X_{t-1}\left(x_{t-2}, \xi_{t-1}\right)
$$
For $\mathrm{t}=\mathrm{T}$,
Since $\mathrm{Q}_{\mathrm{T}+1}(\cdot)=0, \quad \mathrm{Q}_{\mathrm{T}}\left(\mathrm{x}_{\mathrm{T}-1}, \xi_{\mathrm{T}}\right)=\widehat{\mathrm{Q}}_{\mathrm{T}}\left(\mathrm{x}_{\mathrm{T}-1}, \xi_{\mathrm{T}}\right)$
Using Theorem 1, we have the following generalization bound for a fixed $\mathrm{x}_{\mathrm{T}-1} \in \mathcal{X}_{\mathrm{T}-1}\left(\mathrm{x}_{\mathrm{T}-2}, \xi_{\mathrm{T}-1}\right)$.
$\forall \mathrm{x}_{\mathrm{T}-1} \in \mathcal{X}_{\mathrm{T}-1}\left(\mathrm{x}_{\mathrm{T}-2}, \xi_{\mathrm{T}-1}\right), \forall \xi_{\mathrm{T}-1} \in \Xi_{\mathrm{T}-1}^{\mathrm{N}}$
$$
\operatorname{Prob}\left(\left|\mathbb{E}\left[\mathrm{Q}_{\mathrm{T}}\left(\mathrm{x}_{\mathrm{T}-1}, \tilde{\xi}_{\mathrm{T}}\right) \mid \xi_{\mathrm{T}-1}\right]-\widehat{\mathbb{E}}\left[\widehat{\mathrm{Q}}_{\mathrm{T}}\left(\mathrm{x}_{\mathrm{T}-1}, \tilde{\xi}_{\mathrm{T}}\right) \mid \xi_{\mathrm{T}-1}\right]\right| \leq \phi_{\mathrm{T}}\right) \geq 1-\delta_{\mathrm{T}}
$$
where $\phi_{\mathrm{T}}=\sqrt{\frac{\mathbb{V}\left[\mathrm{Q}_{\mathrm{T}}\left(\mathrm{x}_{\mathrm{T}-1}, \tilde{\xi}_{\mathrm{T}}\right) \mid \xi_{\mathrm{T}-1}\right]}{\mathrm{Nh}_{\mathrm{N}}^{\mathrm{p}}\left(\xi_{\mathrm{T}-1}\right)(1+\mathrm{o}(1))} \log \left(\frac{1}{\delta_{\mathrm{T}}}\right)}$



